Benchmarking Composed Image Retrieval for Applied Earth Observation

Remote sensing composed image retrieval (RSCIR) enables search in large satellite image archives using composed queries that combine a reference image with a textual modifier. Although RSCIR offers a flexible interface for expressing targeted retrieval intent, the transferability of modern composition methods to Earth observation (EO) imagery and their relevance to operational EO workflows remain underexplored. We address this gap through a unified benchmark and an application-oriented study. First, we systematically adapt and evaluate representative composed image retrieval methods with six vision-language backbones on PatternCom under a standardized protocol, analyzing their behavior across backbones, composition strategies, and query types. Second, we introduce xView2-CIR, a change-centric dataset for disaster and damage monitoring, where retrieval is conditioned on scene identity and a target post-event state. Our results show that training-free composition methods provide strong and scalable baselines for EO retrieval, while change-centric retrieval presents different challenges from attribute-based retrieval, particularly due to the need to preserve scene identity. Overall, this study establishes a practical benchmark for RSCIR and positions composed retrieval as a complementary tool for remote sensing image retrieval, archive exploration, and change analysis. The dataset and code are available at https://github.com/billpsomas/rscir.

==> tab/ablation_freq_text.tex <==
\begin{table}[tbp]
  \caption{\emph{TODO} TODO.}
  \centering
  \scriptsize
  %— first sub‐table —
  \begin{minipage}[t]{.48\textwidth}
    \centering
    \begin{tabular}{ccccccc}
      \toprule
      \diagbox[innerwidth=4em,height=2em]{$m$}{$k$}
        & 10 & 50 & 100 & 200 & 500 & 1000 \\
      \midrule
      1  & \cellcolor[HTML]{EA9999}25.1 & \cellcolor[HTML]{F8DFDF}28.0 &  
           \cellcolor[HTML]{EA9999}25.1 & \cellcolor[HTML]{F8DFDF}28.0 &
           \cellcolor[HTML]{EA9999}25.1 & \cellcolor[HTML]{F8DFDF}28.0 \\
      3  & \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{99C884}31.5 &
           \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{99C884}31.5 &
           \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{99C884}31.5 \\
      7  & \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{93C47D}31.6 &
           \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{93C47D}31.6 &
           \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{93C47D}31.6 \\
      15 & \cellcolor[HTML]{F6FAF4}29.5 & \cellcolor[HTML]{BEDCB1}30.7 &
           \cellcolor[HTML]{F6FAF4}29.5 & \cellcolor[HTML]{BEDCB1}30.7 &
           \cellcolor[HTML]{F6FAF4}29.5 & \cellcolor[HTML]{BEDCB1}30.7 \\
      \bottomrule
    \end{tabular}

    \\[1ex]\textbf{(a)}
  \end{minipage}%
  \hfill
  %— second sub‐table (identical) —
  \begin{minipage}[t]{.48\textwidth}
    \centering
    \begin{tabular}{ccccccc}
      \toprule
      \diagbox[innerwidth=4em,height=2em]{$m$}{$k$}
        & 10 & 50 & 100 & 200 & 500 & 1000 \\
      \midrule
      1  & \cellcolor[HTML]{EA9999}25.1 & \cellcolor[HTML]{F8DFDF}28.0 &  
           \cellcolor[HTML]{EA9999}25.1 & \cellcolor[HTML]{F8DFDF}28.0 &
           \cellcolor[HTML]{EA9999}25.1 & \cellcolor[HTML]{F8DFDF}28.0 \\
      3  & \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{99C884}31.5 &
           \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{99C884}31.5 &
           \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{99C884}31.5 \\
      7  & \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{93C47D}31.6 &
           \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{93C47D}31.6 &
           \cellcolor[HTML]{F4F9F2}29.6 & \cellcolor[HTML]{93C47D}31.6 \\
      15 & \cellcolor[HTML]{F6FAF4}29.5 & \cellcolor[HTML]{BEDCB1}30.7 &
           \cellcolor[HTML]{F6FAF4}29.5 & \cellcolor[HTML]{BEDCB1}30.7 &
           \cellcolor[HTML]{F6FAF4}29.5 & \cellcolor[HTML]{BEDCB1}30.7 \\
      \bottomrule
    \end{tabular}

    \\[1ex]\textbf{(b)}
  \end{minipage}

  \label{tab:freedom_joint_ablation}
\end{table}

==> tab/ablation_freq_text2.tex <==
% Place this after defining \gradientfreedom and setting:
% \newcommand*{\minvalaverage}{26.71}
% \newcommand*{\maxvalaverage}{40.75}

\begin{table}[t]
  \caption{\emph{Joint hyperparameter search for \oursnew,} using CLIP LAION-2B, measured in attribute modification average mAP (\%). (a) Joint sweep over the number of proxy images ($k$) and merged labels ($m$), keeping $n{=}1$. (b) Sweep over the number of retrieved labels per proxy ($n$), with $m{=}7$ fixed.}
  \label{tab:freedom_final_ablation}
  \centering
  \scriptsize
  \begin{minipage}[t]{.48\textwidth}
    \centering
    \begin{tabular}{ccccccc}
      \toprule
      \diagbox[innerwidth=4em,height=2em]{$m$}{$k$}
        & 10 & 50 & 100 & 200 & 500 & 1000 \\
      \midrule
      1   & \gradientfreedommk{29.77} & \gradientfreedommk{30.18} & \gradientfreedommk{30.41} & \gradientfreedommk{30.36} & \gradientfreedommk{29.49} & \gradientfreedommk{26.71} \\
      3   & \gradientfreedommk{33.09} & \gradientfreedommk{34.27} & \gradientfreedommk{34.62} & \gradientfreedommk{34.87} & \gradientfreedommk{34.59} & \gradientfreedommk{30.99} \\
      7   & \gradientfreedommk{33.45} & \gradientfreedommk{34.89} & \gradientfreedommk{35.29} & \gradientfreedommk{35.58} & \gradientfreedommk{35.68} & \gradientfreedommk{33.29} \\
      15  & \gradientfreedommk{33.45} & \gradientfreedommk{34.82} & \gradientfreedommk{35.19} & \gradientfreedommk{35.45} & \gradientfreedommk{35.61} & \gradientfreedommk{33.68} \\
      \bottomrule
    \end{tabular}
    \\[1ex] \textbf{(a)} \textit{Ablation over $k$ and $m$ ($n=1$ fixed)}
  \end{minipage}%
  \vspace{3pt}
  \begin{minipage}[t]{.48\textwidth}
    \centering
    \begin{tabular}{ccccccc}
      \toprule
      \diagbox[innerwidth=4em,height=2em]{$k$}{$n$}
        & 1 & 2 & 3 & 5 & 7 & 9 \\
      \midrule
      50   & \gradientfreedomkn{34.89} & \gradientfreedomkn{36.84} & \gradientfreedomkn{37.89} & \gradientfreedomkn{38.82} & \gradientfreedomkn{39.39} & \gradientfreedomkn{39.51} \\
      100  & \gradientfreedomkn{35.29} & \gradientfreedomkn{37.33} & \gradientfreedomkn{38.45} & \gradientfreedomkn{39.32} & \gradientfreedomkn{39.87} & \gradientfreedomkn{38.69} \\
      200  & \gradientfreedomkn{35.58} & \gradientfreedomkn{37.68} & \gradientfreedomkn{38.88} & \gradientfreedomkn{39.77} & \gradientfreedomkn{40.25} & \gradientfreedomkn{40.36} \\
      500  & \gradientfreedomkn{35.68} & \gradientfreedomkn{37.90} & \gradientfreedomkn{39.02} & \gradientfreedomkn{40.29} & \gradientfreedomkn{40.75} & \gradientfreedomkn{40.72} \\
      \bottomrule
    \end{tabular}
    \\[1ex] \textbf{(b)} \textit{Ablation over $n$ ($m$ fixed to best $= 7$)}
  \end{minipage}
\end{table}

==> tab/compodiff_tuning.tex <==
\begin{table*}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{cccccccccc}
\toprule
Model & Color & Context & Density & Existence & Quantity & Shape & Average & \# Timesteps & Source Weight \\
\midrule
CompoDiff & 13.05 & 6.48 & 6.59 & 14.40 & 1.16 & 10.00 & 8.61 & 10 & 0.1 \\
CompoDiff & -    & -    & -    & -     & -    & -     & -    & 20 & 0.1 \\
CompoDiff & -    & -    & -    & -     & -    & -     & -    & 30 & 0.1 \\
CompoDiff & 16.87 & 8.96 & 11.55 & 19.64 & 5.08 & 18.80 & 13.48 & 10 & 0.2 \\
CompoDiff & 13.38 & 8.39 & 9.32 & 20.07 & 3.17 & 18.08 & 12.07 & 20 & 0.2 \\
CompoDiff & 12.94 & 8.45 & 8.84 & 20.12 & 2.83 & 17.83 & 11.84 & 30 & 0.2 \\
CompoDiff & 20.36 & 11.38 & 15.31 & 21.34 & 9.12 & 23.31 & 16.80 & 10 & 0.3 \\
CompoDiff & 18.27 & 10.74 & 13.14 & 21.56 & 7.06 & 22.58 & 15.56 & 20 & 0.3 \\
CompoDiff & 17.83 & 10.75 & 12.44 & 22.14 & 6.80 & 22.32 & 15.38 & 30 & 0.3 \\
CompoDiff & 20.59 & 12.67 & 17.57 & 21.98 & 10.23 & 22.31 & 17.56 & 10 & 0.4 \\
CompoDiff & 19.62 & 12.07 & 16.22 & 22.34 & 9.12 & 21.73 & 16.85 & 20 & 0.4 \\
CompoDiff & 19.33 & 11.85 & 15.63 & 22.11 & 8.89 & 21.58 & 16.57 & 30 & 0.4 \\
CompoDiff & 18.51 & 12.19 & 18.74 & 21.49 & 10.39 & 20.41 & 16.96 & 10 & 0.5 \\
CompoDiff & 17.97 & 11.76 & 18.06 & 21.81 & 9.65 & 20.08 & 16.56 & 20 & 0.5 \\
CompoDiff & 17.90 & 11.65 & 17.80 & 21.87 & 9.52 & 19.98 & 16.45 & 30 & 0.5 \\
CompoDiff & 16.65 & 11.39 & 18.85 & 21.27 & 10.16 & 18.86 & 16.20 & 10 & 0.6 \\
CompoDiff & 16.46 & 11.09 & 18.71 & 21.35 & 9.78 & 18.63 & 16.00 & 20 & 0.6 \\
CompoDiff & 16.42 & 11.11 & 18.59 & 21.43 & 9.70 & 18.58 & 15.97 & 30 & 0.6 \\
\bottomrule
\end{tabular}
\caption{Hyperparameter tuning of CompoDiff using SkyCLIP-50 across number of diffusion timesteps and source weight. Average retrieval performance is reported across six attribute types.}
\label{tab:compodiff_hyperparams}
\end{table*}

==> tab/dataset_old.tex <==
\begin{table}[htbp]
\scriptsize
\renewcommand\theadfont{\scriptsize}
\centering
\caption{\emph{Statistics of all the attributes of} \dataset, the first RSCIR benchmark.}
\begin{tabular}{ccccc}
\toprule
\Th{Attribute} &
\Th{Class}  &
\Th{Value} &
\Th{\#Positives}    &
\Th{\#Queries}   \\
\midrule

\multirow{11}{*}{color} & \multirow{2}{*}{airplane} & \texttt{white} & 672 & 53 \\ 
& & \texttt{purple} & 53 & 672 \\ \cmidrule{2-5}

& \multirow{2}{*}{nursing home} & \texttt{white} & 85 & 383 \\ 
& & \texttt{gray} & 383 & 85 \\ \cmidrule{2-5}

& \multirow{2}{*}{crosswalk} & \texttt{white} & 412 & 388 \\
& & \texttt{yellow} & 388 & 412 \\ \cmidrule{2-5}

& \multirow{5}{*}{tennis court} & \texttt{blue} & 339 & 287 \\
& & \texttt{brown} & 2 & 624 \\ 
& & \texttt{gray} & 50 & 576 \\
& & \texttt{green} & 211 & 415 \\
& & \texttt{red} & 24 & 602 \\ \midrule

\multirow{2}{*}{context} & \multirow{2}{*}{bridge} & \texttt{concrete} & 800 & 800 \\ 
& & \texttt{water} & 800 & 800 \\

\midrule
\multirow{2}{*}{density} & \multirow{2}{*}{residential} & sparse & 800 & 800 \\ & & dense & 800 & 800 \\ \midrule
\multirow{4}{*}{existence} & \multirow{2}{*}{parking} & with cars & 947 & 653 \\ & & without cars & 653 & 947 \\ 
 & \multirow{2}{*}{pier} & with boats & 1345 & 255 \\
& & without boats & 255 & 1345 \\ \midrule
\multirow{13}{*}{quantity}  & \multirow{4}{*}{storage tank} & one & 356 & 261 \\
& & two & 119 & 498 \\ 
& & three & 65 & 552 \\
& & four & 77 & 540 \\
 & \multirow{4}{*}{wast. tr. plant} & one & 724 & 78 \\
& & two & 44 & 758 \\ 
& & three & 10 & 792 \\
& & four & 24 & 778 \\
 & \multirow{5}{*}{basketball court} & one & 340 & 383 \\
& & two & 286 & 437 \\ 
& & three & 21 & 702 \\
& & half & 61 & 662 \\
& & two-halfs & 15 & 708 \\   \midrule
\multirow{7}{*}{shape} & \multirow{3}{*}{swimming pool} & rectangular & 261 & 299 \\ 
& & oval & 52 & 508 \\ 
& & kidney-shaped & 247 & 313 \\ 
& \multirow{2}{*}{river} & curved & 177 & 623 \\
& & straight & 623 & 177 \\
& \multirow{2}{*}{road} & cross & 800 & 800 \\
& & round & 800 & 800 \\

\bottomrule
\end{tabular}
\label{tab:dataset}
\end{table}

==> tab/retrieval_old.tex <==

\begin{figure*}
\scriptsize
\centering
\setlength{\tabcolsep}{1.2pt}
\newcommand{\sz}{1.5cm}
\makebox[\linewidth]{
\begin{tabular}{c ccc@{\hspace{4pt}}|@{\hspace{4pt}}ccc@{\hspace{4pt}}|@{\hspace{4pt}}ccc}

%--------------------------------------------
% Image-only
%--------------------------------------------
\multirow{17}{*}{\makecell[c]{(a)\\Image-only}\hspace{2em}}
& Query Image & 1 & 2 
& Query Image & 1 & 2 
& Query Image & 1 & 2 \\

&\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/airplane743.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_airplane743_query_text_purple_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_airplane743_query_text_purple_rank3.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/overpass353.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_overpass353_query_text_water_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_overpass353_query_text_water_rank3.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/sparseresidential245.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_sparseresidential245_query_text_dense_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_sparseresidential245_query_text_dense_rank3.png} \\

&Query Text: &  &  &
Query Text: &  &  &
Query Text: &  &  \\
\vspace{1em}
&\texttt{\textcolor{textquerycolor}{purple}} &  &  &
\texttt{\textcolor{textquerycolor}{water}} &  &  &
\texttt{\textcolor{textquerycolor}{dense}} &  &  \\

&\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/parkinglot373.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_parkinglot373_query_text_empty_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_parkinglot373_query_text_empty_rank3.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/storagetank244.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_storagetank244_query_text_one_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_storagetank244_query_text_one_rank3.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/swimmingpool270.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_swimmingpool270_query_text_rectangular_rank4.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/image-only/query_image_swimmingpool270_query_text_rectangular_rank6.png} \\

&Query Text: &  &  &
Query Text: &  &  &
Query Text: &  &  \\
\vspace{2em}
&\texttt{\textcolor{textquerycolor}{empty}} &  &  &
\texttt{\textcolor{textquerycolor}{one}} &  &  &
\texttt{\textcolor{textquerycolor}{rectangular}} &  &  \\

%--------------------------------------------
% Text-only
%--------------------------------------------
\multirow{17}{*}{\makecell[c]{(b)\\Text-only}\hspace{2em}}
& Query Image & 1 & 2 
& Query Image & 1 & 2 
& Query Image & 1 & 2 \\

&\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/airplane743.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_airplane743_query_text_purple_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_airplane743_query_text_purple_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/overpass353.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_overpass353_query_text_water_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_overpass353_query_text_water_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/sparseresidential245.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_sparseresidential245_query_text_dense_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_sparseresidential245_query_text_dense_rank2.png} \\

&Query Text: &  &  &
Query Text: &  &  &
Query Text: &  &  \\
\vspace{1em}
&\texttt{\textcolor{textquerycolor}{purple}} &  &  &
\texttt{\textcolor{textquerycolor}{water}} &  &  &
\texttt{\textcolor{textquerycolor}{dense}} &  &  \\

&\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/parkinglot373.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_parkinglot373_query_text_empty_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_parkinglot373_query_text_empty_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/storagetank244.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_storagetank244_query_text_one_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_storagetank244_query_text_one_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/swimmingpool270.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_swimmingpool270_query_text_rectangular_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/text-only/query_image_swimmingpool270_query_text_rectangular_rank2.png} \\

&Query Text: &  &  &
Query Text: &  &  &
Query Text: &  &  \\
\vspace{2em}
&\texttt{\textcolor{textquerycolor}{empty}} &  &  &
\texttt{\textcolor{textquerycolor}{one}} &  &  &
\texttt{\textcolor{textquerycolor}{rectangular}} &  &  \\

%--------------------------------------------
% WeiCom
%--------------------------------------------
\multirow{17}{*}{\makecell[c]{(c)\\WeiCom}\hspace{2em}}
& Query Image & 1 & 2 
& Query Image & 1 & 2 
& Query Image & 1 & 2 \\

&\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/airplane743.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_airplane743_query_text_purple_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_airplane743_query_text_purple_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/overpass353.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_overpass353_query_text_water_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_overpass353_query_text_water_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/sparseresidential245.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_sparseresidential245_query_text_dense_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_sparseresidential245_query_text_dense_rank2.png} \\

&Query Text: &  &  &
Query Text: &  &  &
Query Text: &  &  \\
\vspace{1em}
&\texttt{\textcolor{textquerycolor}{purple}} &  &  &
\texttt{\textcolor{textquerycolor}{water}} &  &  &
\texttt{\textcolor{textquerycolor}{dense}} &  &  \\

&\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/parkinglot373.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_parkinglot373_query_text_empty_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_parkinglot373_query_text_empty_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/storagetank244.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_storagetank244_query_text_four_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_storagetank244_query_text_four_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/swimmingpool270.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_swimmingpool270_query_text_oval_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/weicom/query_image_swimmingpool270_query_text_oval_rank2.png} \\

&Query Text: &  &  &
Query Text: &  &  &
Query Text: &  &  \\
\vspace{2em}
&\texttt{\textcolor{textquerycolor}{empty}} &  &  &
\texttt{\textcolor{textquerycolor}{one}} &  &  &
\texttt{\textcolor{textquerycolor}{rectangular}} &  &  \\

%--------------------------------------------
% FreeDom
%--------------------------------------------
\multirow{17}{*}{\makecell[c]{(d)\\FreeDom}\hspace{2em}}
& Query Image & 1 & 2 
& Query Image & 1 & 2 
& Query Image & 1 & 2 \\

&\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/airplane743.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_airplane743_query_text_purple_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_airplane743_query_text_purple_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/overpass353.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_overpass353_query_text_water_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_overpass353_query_text_water_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/sparseresidential245.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_sparseresidential245_query_text_dense_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_sparseresidential245_query_text_dense_rank3.png} \\

&Query Text: &  &  &
Query Text: &  &  &
Query Text: &  &  \\
\vspace{1em}
&\texttt{\textcolor{textquerycolor}{purple}} &  &  &
\texttt{\textcolor{textquerycolor}{water}} &  &  &
\texttt{\textcolor{textquerycolor}{dense}} &  &  \\

&\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/parkinglot373.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_parkinglot373_query_text_empty_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_parkinglot373_query_text_empty_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/storagetank244.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_storagetank244_query_text_one_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_storagetank244_query_text_one_rank2.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/queries/swimmingpool270.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_swimmingpool270_query_text_rectangular_rank1.png} &
\includegraphics[width=\sz,height=\sz]{fig/retrieval/freedom/query_image_swimmingpool270_query_text_rectangular_rank2.png} \\

&Query Text: &  &  &
Query Text: &  &  &
Query Text: &  &  \\

&\texttt{\textcolor{textquerycolor}{empty}} &  &  &
\texttt{\textcolor{textquerycolor}{one}} &  &  &
\texttt{\textcolor{textquerycolor}{rectangular}} &  &  \\

\end{tabular}
}
\caption{\emph{Qualitative retrieval results} of composed image retrieval on \dataset using four different methods with OpenAI CLIP. Each column triad shows the top-2 retrieved results across distinct attribute modifications: color, context, density, existence, quantity, and shape (from left to right).}
\label{fig:retrievals}
\end{figure*}
%------------------------------------------------------------------------------

==> tab/weicom_lambda_ablation.tex <==
\begin{table*}[htbp]
\caption{\emph{The impact of the modality control parameter $\lambda$ on} \ours using RemoteCLIP, measured in attribute modification mAP (\%).}
\centering
\scriptsize
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{lccccccccccc}
\toprule
$\lambda$ & 0 & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 \\
\midrule
%Shape     & \gradientshape{17.7} & \gradientshape{36.7} & \gradientshape{35.2} & \gradientshape{33.1} & \gradientshape{30.4} & \gradientshape{27.0} & \gradientshape{23.1} & \gradientshape{18.4} & \gradientshape{12.8} & \gradientshape{7.1} & \gradientshape{2.1} \\
%Color     & \gradientcolor{9.3} & \gradientcolor{58.3} & \gradientcolor{60.0} & \gradientcolor{60.2} & \gradientcolor{59.9} & \gradientcolor{59.4} & \gradientcolor{58.7} & \gradientcolor{57.9} & \gradientcolor{56.9} & \gradientcolor{55.3} & \gradientcolor{34.2} \\
%Density   & \gradientdensity{15.1} & \gradientdensity{23.3} & \gradientdensity{29.5} & \gradientdensity{34.0} & \gradientdensity{37.4} & \gradientdensity{39.9} & \gradientdensity{41.6} & \gradientdensity{42.0} & \gradientdensity{40.7} & \gradientdensity{35.9} & \gradientdensity{22.2} \\
%Quantity  & \gradientquantity{8.3} & \gradientquantity{33.3} & \gradientquantity{36.1} & \gradientquantity{37.3} & \gradientquantity{37.8} & \gradientquantity{38.1} & \gradientquantity{38.0} & \gradientquantity{37.7} & \gradientquantity{36.9} & \gradientquantity{35.0} & \gradientquantity{15.2} \\ \midrule
%Average   & \gradientaverage{12.6} & \gradientaverage{37.9} & \gradientaverage{40.2} & \gradientaverage{41.1} & \gradientaverage{41.4} & \gradientaverage{41.1} & \gradientaverage{40.3} & \gradientaverage{39.0} & \gradientaverage{36.8} & \gradientaverage{33.3} & \gradientaverage{18.4} \\
Color     & \gradientcolor{14.5} & \gradientcolor{55.3} & \gradientcolor{53.0} & \gradientcolor{49.6} & \gradientcolor{46.4} & \gradientcolor{43.7} & \gradientcolor{41.0} & \gradientcolor{38.2} & \gradientcolor{35.0} & \gradientcolor{30.4} & \gradientcolor{10.8} \\
Context     & \gradientcontext{6.6}     & \gradientcontext{13.3}     & \gradientcontext{20.2}     & \gradientcontext{25.7}     & \gradientcontext{29.5}     & \gradientcontext{31.5}     & \gradientcontext{31.6}     & \gradientcontext{29.6}     & \gradientcontext{24.8}     & \gradientcontext{16.9}     & \gradientcontext{8.9} \\
Density     & \gradientdensity{15.1}     & \gradientdensity{23.3}     & \gradientdensity{29.5}     & \gradientdensity{34.0}     & \gradientdensity{37.4}     & \gradientdensity{39.9}     & \gradientdensity{41.6}     & \gradientdensity{42.0}     & \gradientdensity{40.7}     & \gradientdensity{35.9}     & \gradientdensity{22.2} \\
Existence     & \gradientexistence{13.1}     & \gradientexistence{14.2}     & \gradientexistence{14.5}     & \gradientexistence{15.0}     & \gradientexistence{15.0}     & \gradientexistence{14.9}     & \gradientexistence{14.6}     & \gradientexistence{13.8}     & \gradientexistence{12.5}     & \gradientexistence{10.3}     & \gradientexistence{7.0} \\
Quantity     & \gradientquantity{7.0}     & \gradientquantity{17.6}     & \gradientquantity{18.9}    & \gradientquantity{19.7}     & \gradientquantity{20.2}     & \gradientquantity{20.5}     & \gradientquantity{20.8}     & \gradientquantity{20.9}     & \gradientquantity{20.8}     & \gradientquantity{20.1}     & \gradientquantity{8.3} \\
Shape     & \gradientshape{15.2}     & \gradientshape{23.8}     & \gradientshape{24.7}     & \gradientshape{26.2}     & \gradientshape{28.0}     & \gradientshape{29.8}     & \gradientshape{31.2}     & \gradientshape{32.0}     & \gradientshape{32.0}     & \gradientshape{31.3}     & \gradientshape{24.1} \\
\midrule
Average     & \gradientaverage{11.9}     & \gradientaverage{24.6}     & \gradientaverage{26.8}     & \gradientaverage{28.4}     & \gradientaverage{29.4}     & \gradientaverage{30.0}     & \gradientaverage{30.1}     & \gradientaverage{29.4}     & \gradientaverage{27.6}     & \gradientaverage{24.2}     & \gradientaverage{13.6} \\


\bottomrule
\end{tabular}
}
\label{tab:ablation}
\end{table*}

==> tex/abstract.tex <==
Remote sensing composed image retrieval (RSCIR) enables search in large satellite image archives using composed queries that combine a reference image with a textual modifier. Although RSCIR offers a flexible interface for expressing targeted retrieval intent, the transferability of modern composition methods to Earth observation (EO) imagery and their relevance to operational EO workflows remain underexplored. We address this gap through a unified benchmark and an application-oriented study. First, we systematically adapt and evaluate representative composed image retrieval methods with six vision-language backbones on PatternCom under a standardized protocol, analyzing their behavior across backbones, composition strategies, and query types. Second, we introduce xView2-CIR, a change-centric dataset for disaster and damage monitoring, where retrieval is conditioned on scene identity and a target post-event state. Our results show that training-free composition methods provide strong and scalable baselines for EO retrieval, while change-centric retrieval presents different challenges from attribute-based retrieval, particularly due to the need to preserve scene identity. Overall, this study establishes a practical benchmark for RSCIR and positions composed retrieval as a complementary tool for remote sensing image retrieval, archive exploration, and change analysis. %The dataset and code are available at \href{https://github.com/billpsomas/rscir}{https://github.com/billpsomas/rscir}.


==> tex/abstract_old.tex <==
This work introduces and benchmarks composed image retrieval for remote sensing. It enables querying large-scale satellite image archives by combining a query image with a query text, enriching the expressive power over unimodal queries.
%
We present the first benchmark for this task, \dataset, focused on the modification of six attribute types: color, context, density, existence, quantity, and shape. 
%
We conduct an extensive evaluation across six vision-language models—including CLIP, SigLIP, RemoteCLIP, and SkyCLIP—and six state-of-the-art composition methods from computer vision—including Pic2Word, SEARLE, FreeDom, and MagicLens.
%
By ``grounding" these methods to the remote sensing domain, we identify \oursnew as the new state-of-the-art, outperforming the earlier \ours method.
%
Our work fills a gap in remote sensing image retrieval and establishes the first comprehensive benchmark for multimodal compositional search in this domain. Dataset and code: \href{https://github.com/billpsomas/rscir}{https://github.com/billpsomas/rscir}.

==> tex/acknowledgements.tex <==
\noindent\textbf{Acknowledgements:}
Bill was supported by the EU Horizon Europe programme MSCA PF RAVIOLI (No. 101205297).
AWS resources were provided by the National Infrastructures for Research and Technology GRNET and funded by the EU Recovery and Resiliency Facility.

==> tex/extended_related_works.tex <==
\section{Related Work}

\subsection{Composed Image Retrieval (CIR)}
Composed Image Retrieval (CIR) is the task of retrieving an image from a large corpus that matches a given query provided by the user as an image-language pair. Unlike unimodal retrieval tasks such as text-to-text \cite{guo2010research} or image-to-image retrieval \cite{jegou2010improving}, CIR involves both text and visual modalities, making it more complex and requiring robust multimodal understanding. The objective of CIR is to develop a model that can effectively integrate and retrieve information from both textual and visual domains. A key challenge in CIR is learning the interaction between the two modalities and ensuring the retrieval model can generalize across diverse query compositions.

Traditional CIR approaches relied on handcrafted features or late fusion techniques to combine visual and textual information \cite{johnson2015image}. However, these methods often struggled with generalization due to the difficulty of aligning the semantic meaning of images and text. More recent deep learning-based approaches use neural networks to jointly model image and text embeddings \cite{vo2019composing}. These models are often trained using contrastive learning or metric learning techniques, ensuring that semantically similar image-text pairs are closer in the learned feature space. Additionally, large-scale datasets such as CIRR \cite{liu2021image} and Fashion-IQ \cite{guo2019fashion} have facilitated the development of more robust CIR models by providing high-quality compositional image-text pairs.

Recent advancements in multimodal learning, particularly Vision-Language Models (VLMs), have significantly improved performance in CIR by enabling better alignment between textual and visual features \cite{baldrati2023efficient}. These models leverage powerful neural architectures and large-scale pretraining strategies to enhance the ability to capture fine-grained multimodal relationships, which are crucial for effective CIR systems.

\subsection{Vision-Language Models (VLM)}
Vision-Language Models (VLMs) \cite{zhang2024magiclensselfsupervisedimageretrieval} aim to establish a strong correlation between image and text inputs, facilitating better multimodal understanding for various tasks, including retrieval, captioning, and classification. These models are typically trained on large-scale datasets containing paired image-text data and employ a dual-encoder architecture—one encoder for text and another for images. The learned representations are then aligned using contrastive learning or other pre-training objectives.

Foundation models, such as CLIP \cite{radford2021learning} and ALIGN \cite{jia2021scaling}, leverage massive datasets and self-supervised learning techniques to achieve strong zero-shot capabilities. One key objective used in these models is image-text matching, where the global correlation between image features and text features is optimized to enhance retrieval performance \cite{li2022blip}. Additionally, models like BLIP \cite{li2022blip} and ALBEF \cite{li2021align} introduce mechanisms for adaptive image-text alignment, further improving retrieval quality by leveraging fine-grained multimodal interactions.

Modern VLMs employ a variety of architectures and learning strategies. Transformer-based models, such as ViLBERT \cite{lu2019vilbert} and VisualBERT \cite{li2019visualbert}, incorporate self-attention mechanisms to model complex relationships between vision and language modalities. Some approaches integrate object detection modules to extract region-based features, while others utilize end-to-end architectures for direct feature learning \cite{chen2020uniter}. Recent advancements in masked language modeling and multimodal contrastive learning have further enhanced VLM performance, allowing these models to perform robustly in diverse applications, including CIR, image captioning, and visual question answering (VQA).

\subsection{Contrastive Language-Image Pretraining (CLIP)}
Contrastive Language-Image Pretraining (CLIP) \cite{radford2021learning} is a contemporary model designed to learn joint representations of images and text through contrastive learning. Unlike traditional supervised models, CLIP is trained in a multimodal setting using a large-scale dataset of image-text pairs sourced from the internet. The model employs a dual-encoder architecture, where an image encoder and a text encoder are optimized simultaneously using a contrastive loss function. This approach aligns textual and visual embeddings in a shared latent space, enabling effective cross-modal retrieval and classification.

A key advantage of CLIP is its ability to generalize to new tasks without requiring task-specific labeled data. By leveraging large-scale pretraining, CLIP demonstrates strong zero-shot performance across various domains, including image classification, retrieval, and even compositional reasoning \cite{shen2023clip, galassi2023investigating}. Compared to previous vision-language models that required extensive fine-tuning on specific datasets \cite{li2019visualbert, lu2019vilbert}, CLIP's contrastive learning paradigm allows for greater flexibility and adaptability. Moreover, extensions of CLIP, such as CLOOB \cite{mehrer2022cloob}, have been proposed to further refine its contrastive learning framework and enhance retrieval performance by introducing additional regularization techniques.

By integrating large-scale pretraining, contrastive learning, and a diverse dataset of internet-sourced image-text pairs, CLIP represents a significant advancement in vision-language modeling. Its strong performance in retrieval tasks highlights the effectiveness of contrastive pretraining in improving multimodal representations and broadens the potential applications of vision-language models in real-world scenarios.



==> tex/fig_presentation.tex <==
{
%\scriptsize
\footnotesize
\centering
\newcommand{\myg}[1]{\includegraphics[width=0.135\textwidth,valign=c]{#1}}

\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{}ccc@{}}
   
    \mycaption{Query Image} & 
    \mycaption{Query Text} & 
    \mycaption{Retrieved Image} \\
    
    \myg{fig/examples/airplane159.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{purple}}} & 
    \myg{fig/examples/airplane073.jpg} \\
    \mc{3}{(a) Color}\\

    \mc{3}{\vspace{-2.1ex}}\\
    \myg{fig/examples/swimmingpool408.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{circular}}} & 
    \myg{fig/examples/swimmingpool314.jpg} \\

    \mc{3}{(b) Shape
    }\\

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/forest520.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{fine}}} & 
    \myg{fig/examples/forest081.jpg} \\

    \mc{3}{(d) Texture
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/christmastreefarm410.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{dense}}} & 
    \myg{fig/examples/christmastreefarm161.jpg} \\

    \mc{3}{(e) Density
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/airplane388.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{bigger}}} & 
    \myg{fig/examples/airplane697.jpg} \\

    \mc{3}{(c) Size
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/wastewaterplant614.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{four}}} & 
    \myg{fig/examples/wastewaterplant691.jpg} \\

    \mc{3}{(f) Quantity
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/denseresidential690.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{by the sea}}} & 
    \myg{fig/examples/coastalmansion573.jpg} \\

    \mc{3}{(g) Context
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/parkingspace002.jpg} & 
    \fbox{\parbox[c][0.1215\textwidth][c]{0.125\textwidth}{\centering \texttt{with cars}}} & 
    \myg{fig/examples/parkinglot453.jpg} \\

    \mc{3}{(h) Addition
    }\\ 

\end{tabular}
}

==> tex/fig_presentation_col1.tex <==
{
%\scriptsize
\footnotesize
\centering
\newcommand{\myg}[1]{\includegraphics[width=0.26\textwidth,valign=c]{#1}}

\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{}ccc@{}}

    \mycaption{Query} & 
    \mycaption{Query} & 
    \mycaption{Target} \\

    \mycaption{Image} & 
    \mycaption{Text} & 
    \mycaption{Image} \\
    
    \myg{fig/examples/airplane159.jpg} & 
    \fbox{\parbox[c][0.24\textwidth][c]{0.24\textwidth}{\centering \texttt{purple}}} & 
    \myg{fig/examples/airplane073.jpg} \\
    \mc{3}{(a) Color}\\

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/sparseresidential017.jpg} & 
    \fbox{\parbox[c][0.24\textwidth][c]{0.24\textwidth}{\centering \texttt{dense}}} & 
    \myg{fig/examples/denseresidential258.jpg} \\

    \mc{3}{(c) Density
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/wastewaterplant614.jpg} & 
    \fbox{\parbox[c][0.24\textwidth][c]{0.24\textwidth}{\centering \texttt{four}}} & 
    \myg{fig/examples/wastewaterplant691.jpg} \\

    \mc{3}{(e) Quantity
    }\\ 

%    \mc{3}{\vspace{-2.1ex}}\\

%    \myg{fig/examples/airplane388.jpg} & 
%    \fbox{\parbox[c][0.26\textwidth][c]{0.26\textwidth}{\centering \texttt{big}}} & 
%    \myg{fig/examples/airplane697.jpg} \\

%    \mc{3}{(g) Size
%    }\\ 
    
\end{tabular}
}

==> tex/fig_presentation_col2.tex <==
{
\scriptsize
\footnotesize
\centering
\newcommand{\myg}[1]{\includegraphics[width=0.26\textwidth,valign=c]{#1}}

\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{}ccc@{}}
   
    \mycaption{Query} & 
    \mycaption{Query} & 
    \mycaption{Target} \\

    \mycaption{Image} & 
    \mycaption{Text} & 
    \mycaption{Image} \\

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/overpass069.jpg} & 
    \fbox{\parbox[c][0.24\textwidth][c]{0.24\textwidth}{\centering \texttt{water}}} & 
    \myg{fig/examples/bridge307.jpg} \\

    \mc{3}{(b) Context
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\

    \myg{fig/examples/parkingspace002.jpg} & 
    \fbox{\parbox[c][0.24\textwidth][c]{0.24\textwidth}{\centering \texttt{full}}} & 
    \myg{fig/examples/parkinglot453.jpg} \\

    \mc{3}{(d) Existence
    }\\ 

    \mc{3}{\vspace{-2.1ex}}\\
    
    \myg{fig/examples/swimmingpool408.jpg} & 
    \fbox{\parbox[c][0.24\textwidth][c]{0.24\textwidth}{\centering \texttt{oval}}} & 
    \myg{fig/examples/swimmingpool314.jpg} \\

    \mc{3}{(f) Shape
    }\\

%    \mc{3}{\vspace{-2.1ex}}\\

%    \myg{fig/examples/forest520.jpg} & 
%    \fbox{\parbox[c][0.26\textwidth][c]{0.26\textwidth}{\centering \texttt{fine}}} & 
%    \myg{fig/examples/forest081.jpg} \\

%    \mc{3}{(h) Texture
%    }\\ 

\end{tabular}
}
